Projective representations of Hecke groups from Topological quantum field theory

We construct projective (unitary) representations of Hecke groups from the vector spaces associated with the Witten-Reshetikhin-Turaev topological quantum field theory of higher genus surfaces. In particular, we generalize the modular data of Temperley-Lieb-Jones modular categories. We also study some properties of the representation. We show the image group of the representation is infinite at low levels in genus $2$ by explicit computations. We also show the representation is reducible with at least three irreducible summands when the level equals $4l+2$ for $l\geq 1$.

==> symbols.tex <==
\usepackage{amsmath,amsfonts,amssymb,mathtools,amsthm,dsfont}
\usepackage[colorlinks,linkcolor=blue,citecolor=blue]{hyperref}
\usepackage{tikz}
\usetikzlibrary{cd, calc, knots}
\usepackage{xcolor}

\usepackage[utf8]{inputenc}
%\usepackage[notref, notcite]{showkeys}
\usepackage{amsbsy}

\newcommand{\al}{\alpha}

\def\b{\beta}
\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\ep}{\epsilon}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\z}{\zeta}

\newcommand{\et}{\eta}

\newcommand{\te}{\theta}
\newcommand{\Te}{\Theta}

\newcommand{\io}{\iota}

\newcommand{\K}{\kappa}

\newcommand{\n}{\nu}

\newcommand{\x}{\xi}
\newcommand{\X}{\Xi}

\newcommand{\R}{\rho}

\newcommand{\sm}{\sigma}
\newcommand{\Sm}{\Sigma}

\newcommand{\T}{\tau}

\newcommand{\up}{\upsilon}
\newcommand{\Up}{\Upsilon}

\newcommand{\f}{\phi}
\newcommand{\F}{\Phi}

\newcommand{\ch}{\chi}

\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}


\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\op}{\oplus}
\newcommand{\ot}{\otimes}
\newcommand{\bt}{\boxtimes}
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\lrang}[1]{\langle #1\rangle}
\renewcommand{\o}{\otimes}


\newcommand{\sst}{\subset}
\newcommand{\res}[1]{|_{#1}}
\newcommand{\rational}{\mathbb{Q}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\cx}{\mathbb{C}}
\newcommand{\cat}[1]{\mathcal{#1}}
\newcommand{\lie}[1]{\mathfrak{#1}}
\newcommand{\cob}[2]{#1^{-1}#2#1}

\def\Vec{\operatorname{Vec}}
\def\Fun{\operatorname{Fun}}

\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\so}{\mathfrak{so}}
\newcommand{\fm}{\mathfrak{m}}

\newcommand{\BB}{\mathcal{B}}
\newcommand{\BC}{\mathbb{C}}
\newcommand{\BN}{\mathbb{N}}
\newcommand{\BQ}{\mathbb{Q}}
\newcommand{\BZ}{\mathbb{Z}}
\newcommand{\BF}{\mathbb{F}}
\newcommand{\BR}{\mathbb{R}}
\renewcommand{\AA}{\mathcal{A}}
\newcommand{\CC}{{\mathcal{C}}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\ZZ}{\mathcal{Z}}
\newcommand{\EE}{\mathcal{E}}
\def\FF{\mathcal{F}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\VV}{\mathcal{V}}
\def\SS{\mathcal{S}}
\def\MM{\mathcal{M}}
\def\TT{\mathcal{T}}
\newcommand{\OO}{\mathcal{O}}
\def\UU{\mathcal{U}}

\newcommand{\s}{\sigma}
\newcommand{\hs}{{\hat{\sigma}}}
\newcommand{\bs}{[\sigma]}
\newcommand{\ts}{{\tilde{\s}}}

\newcommand{\m}{\mu}
\newcommand{\hm}{{\hat{\mu}}}
\newcommand{\bm}{[\mu]}
\newcommand{\tm}{\tilde{\mu}}


\newcommand{\ld}{\lambda}
\newcommand{\hld}{\hat{\lambda}}
\newcommand{\hl}{{\hat{\ld}}}
\newcommand{\bl}{{[\ld]}}
\newcommand{\Ld}{\Lambda}

\renewcommand{\k}{\kappa}
\newcommand{\hk}{{\hat{\k}}}


\renewcommand{\l}{\ell}

\newcommand{\e}{\varepsilon}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{question}[thm]{Question}
\newtheorem{conj}[thm]{Conjecture}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
%\renewcommand{\theequation}{\thechapter.\arabic{equation}}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{example}[thm]{Example}

\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tH}{{\tilde{H}_{\CC}}}
\newcommand{\ev}{\operatorname{ev}}
\newcommand{\coev}{\operatorname{coev}}
\newcommand{\GL}{\operatorname{GL}}
\def\SL{\operatorname{SL}}
\def\sl{\mathfrak{sl}}
\newcommand{\euler}{\varphi}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\gal}{\operatorname{Gal}}
\newcommand{\irr}{\operatorname{Irr}}
\newcommand{\FPdim}{\operatorname{FPdim}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Real}{\operatorname{Re}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\stab}{\operatorname{Stab}}
\renewcommand{\bot}{\boxtimes}
\newcommand{\Rep}{\operatorname{Rep}}
\newcommand{\diag}{\operatorname{Diag}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\sgn}{\operatorname{sgn}}
\def\span{{\operatorname{span}}}
\newcommand{\herm}[1]{\langle {#1} \rangle}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\PGL}{\operatorname{PGL}}


\newcommand{\ldual}[1]{#1^\ast}
\newcommand{\rdual}[1]{{}^\ast#1}
\newcommand{\lev}[1]{\mathrm{ev}^l_{#1}}
\newcommand{\rightev}[1]{\mathrm{ev}^r_{#1}}
\newcommand{\lcoev}[1]{\mathrm{coev}^l_{#1}}
\newcommand{\rcoev}[1]{\mathrm{coev}^r_{#1}}
\newcommand{\unit}{\mathds{1}}
\newcommand{\twist}[1]{\theta_{#1}}

\newcommand{\1}{\mathds{1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{cyan}{#1}}

\def\GQ{\gal(\bar\BQ)}
\def\svec{\operatorname{sVec}}
\def\W{\mathcal{W}}
\def\sW{{s\mathcal{W}}}
\def\pt{{\operatorname{pt}}}
\def\un{{\operatorname{un}}}
\def\FSexp{{\operatorname{FSexp}}}

\def\Str{{\operatorname{Str}}}
\def\Sp{\operatorname{Sp}}
\def\orb{{\operatorname{Orb}}}
\def\res{{\operatorname{res}}}
\def\spec{{\operatorname{spec}}}

\def\O2{\Omega_2}
\def\zp{\zeta_{p}}


\newcommand{\porb}{
\begin{pmatrix}
\zp^a & & \\
& \ddots &\\
&& \zp^{ar^{2}}
\end{pmatrix}
}

\def\Fib{\operatorname{Fib}}

\def\rev{\operatorname{rev}}
\def\Sem{\operatorname{Sem}}

\newcommand{\2}{\mathds{Y}}
\newcommand{\resnS}{\res_{\BQ(S)}^{\BQ_{n}}}
\newcommand{\qorb}[1]{{[#1]}}

\newcommand{\Zn}[1]{\BZ/{#1}\BZ}
\newcommand{\Znx}[1]{(\BZ/{#1}\BZ)^{\times}}
\newcommand{\Gn}[1]{\gal(\BQ_{#1})}

\newcommand{\td}[1]{\tilde{#1}}
\newcommand{\chtr}{\operatorname{ch}}

\newcommand{\hGn}[1]{\widehat{\gal}(\BQ_{#1})}
\newcommand{\hG}{\widehat{G}}
\newcommand{\hres}{\widehat{\res}}
\def\f2{\varphi_{2}}

\newcommand{\be}{\mathbf{e}}

\newcommand{\GF}[1]{\mathbb{F}_{#1}}
\newcommand{\hGF}[1]{\widehat{\mathbb{F}}^{\times}_{#1}}


\newcommand{\brkt}[1]{\langle #1 \rangle}



\newcommand{\fchi}[1]{f^{\chi_{#1}}}

\newcommand{\Nm}{\pmb{N}}

\newcommand{\NN}{\mathcal{N}}

\newcommand{\zz}{\zeta_{32}}



\renewcommand{\mod}{\operatorname{mod}}

\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\jac}[1]{\left( {#1} \right)_{J}}

\renewcommand{\AA}{\mathcal{A}}
\def\Tr{{\operatorname{tr}}}
\def\ob{{\operatorname{ob}}}
\newcommand{\sqdim}[1]{{\sqrt{\dim(#1)}}}
\def\Vs{{\operatorname{Vec}}}
\newcommand{\bte}{{\boxtimes_{\EE}}}



